Towards concept analysis in categories: limit inferior as algebra, limit superior as coalgebra

While computer programs and logical theories begin by declaring the concepts of interest, be it as data types or as predicates, network computation does not allow such global declarations, and requires *concept mining* and *concept analysis* to extract shared semantics for different network nodes. Powerful semantic analysis systems have been the drivers of nearly all paradigm shifts on the web. In categorical terms, most of them can be described as bicompletions of enriched matrices, generalizing the Dedekind-MacNeille-style completions from posets to suitably enriched categories. Yet it has been well known for more than 40 years that ordinary categories themselves in general do not permit such completions. Armed with this new semantical view of Dedekind-MacNeille completions, and of matrix bicompletions, we take another look at this ancient mystery. It turns out that simple categorical versions of the *limit superior* and *limit inferior* operations characterize a general notion of Dedekind-MacNeille completion, that seems to be appropriate for ordinary categories, and boils down to the more familiar enriched versions when the limits inferior and superior coincide. This explains away the apparent gap among the completions of ordinary categories, and broadens the path towards categorical concept mining and analysis, opened in previous work.

==> PIC/spectral.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 13 18:40:59 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="90" y-min="2.5" y-max="52.5" auto-bounding="true">
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(20,40);(20,40);(80,40);(80,40)"
%	 />
%<multicurve stroke-width= "0.2"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "double-head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(85,35);(85,35);(75,10);(75,10)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\alice$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\bob$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,42.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOneBack$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(82.5,52.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(77,5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\intoOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,2.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\intoOneBack$
%</text>
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(30,5);(30,5);(70,5);(70,5)"
%	 />
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 left-arrow= "reverse-head"
%	 points= "(80,10);(80,10);(90,35);(90,35)"
%	 />
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "double-head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(10,35);(10,35);(20,10);(20,10)"
%	 />
%<multicurve stroke-width= "0.2"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 left-arrow= "reverse-head"
%	 points= "(25,10);(25,10);(15,35);(15,35)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(87,23)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\rightout$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,23)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\rightin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,22)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\leftin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13,23)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\leftout$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(90,52.5)
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(20,40)(80,40)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->>}(85,35)(75,10)
\rput(10,40){$\alice$}
\rput(90,40){$\bob$}
\rput(50,42.5){$\msgOne$}
\rput(24,5){$\msgOneBack$}
\rput[b](82.5,52.5){}
\rput(77,5){$\intoOne$}
\rput(50,2.5){$\intoOneBack$}
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(30,5)(70,5)
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{>->}(80,10)(90,35)
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->>}(10,35)(20,10)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{>->}(25,10)(15,35)
\rput[l](87,23){$\rightout$}
\rput[r](79,23){$\rightin$}
\rput[l](22,22){$\leftin$}
\rput[r](13,23){$\leftout$}
\end{pspicture}

